Deepfake Videos in the Wild: Analysis and Detection

AI-manipulated videos, commonly known as deepfakes, are an emerging problem. Recently, researchers in academia and industry have contributed several (self-created) benchmark deepfake datasets, and deepfake detection algorithms. However, little effort has gone towards understanding deepfake videos in the wild, leading to a limited understanding of the real-world applicability of research contributions in this space. Even if detection schemes are shown to perform well on existing datasets, it is unclear how well the methods generalize to real-world deepfakes. To bridge this gap in knowledge, we make the following contributions: First, we collect and present the largest dataset of deepfake videos in the wild, containing 1,869 videos from YouTube and Bilibili, and extract over 4.8M frames of content. Second, we present a comprehensive analysis of the growth patterns, popularity, creators, manipulation strategies, and production methods of deepfake content in the real-world. Third, we systematically evaluate existing defenses using our new dataset, and observe that they are not ready for deployment in the real-world. Fourth, we explore the potential for transfer learning schemes and competition-winning techniques to improve defenses.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle


==> body.tex <==
\section{Introduction}
fill pointers 

\bimal{Need to mention key research questions/goals here. Next few sections are a lot of a background, so important to establish this early on.}


\section{Background}
\subsection{Deepfake Videos}
\bimal{This should be a short section. Key points: 1. our definition of deepfake videos. 2. what types of deepfakes we focus on? 3. Give brief history of first deepfakes/evolution on the web, but mention that core methods were developed by the academic community (is that correct?) 4. Mention simultaneous progress in the web and academic community }
Our focus is on videos of human faces...
The techniques of manipulating multimedia content are extensively proposed and created into application, including both traditional image altering tools and deep learning based forgery techniques. Recent advances in deep learning have led to a giant leap of multimedia content realism, and AI-synthesized images and videos can be vividly generated to deceive human eyes with the help of deep neural networks such as AutoEncoder. Deepfake, which is face-swapping technique, appeared in late 2017 in Reddit to replace the face of a targeted person with the face of someone else, e.g., a celebrity’s face. Meanwhile, applications such as FakeApp and DeepFaceLab based on Deepfake are quickly created by the community. Such techniques have profoundly threatened the authenticity of multimedia contents and increase researchers’ interests in digital forensics.\bimal{this para is saying a lot of things, and is all over the place. what are the key points you want to make?}





\subsection{Methods for Generating Deepfakes}
% Begin with quick discussion origins of Deepfakes: see reddit user, uwashington obama video. Mention names of initial tools like FakeApp.
A wide variety of deepfake-generation tools and methodologies have been released by both academia and the web community of deepfake enthusiasts. We provide a brief summary of these tools and methodologies below. In order to provide common terminology, we adopt the following convention: the \textit{source} face is the face to be swapped in, and the \textit{target} face is the face that will be replaced, but whose expression and pose will be retained. \todo{For each generation method explain: a) creation date/venue if available b) creator/owner/maintainer c) core neural architecture e) project status.}
\bimal{Give a few samples of high quality videos produced in the wild}

\noindent\textbf{Web community.} \bimal{1. Mainly focus on methods for which have videos collected. 2. But mention that there are a large number of videos for which we have no idea about the method. 3. put every other method into a miscellaneous/other category. 4. about each method, mention when the tool was available, the method used, and comment on the quality/level of tuning/variation possible. Basically we want to give people a sense for how sophisticated the tools are.} This category comprises tools and methodologies built entirely by programmers, VFX artists and other technically inclined individuals. For each tool/method, we detail the creation timeline, owners, core neural architecture, extra features and maintenance status. 


\begin{enumerate}
    \item \textbf{FaceSwap}: FaceSwap was created in 2017. It is not owned by a individual, but is maintained by online users \textit{torzdf, kvrooman, kilyroythethird, Clorr, andexina, gdunstone, brylanlyon} and  \textit{Ganonmaster}. FaceSwap employs a core neural architecture for face-swapping, which employs two deep auto-encoders. Each auto-encoder is trained independently (using a mean absolute error or SSIM reconstruction loss) to reconstruct the corresponding face from the latent variable. The key architectural modification that enables face-swapping is that the auto-encoders share a single encoder. This ensures that the encoder disentangles facial identity from facial expression. To swap a face, the source individual's face is fed into the shared encoder, and the target individual's decoder is used to decode the latent representation. The result is the swapped face i.e. with the target's identity, but the source's facial expression. FaceSwap offers 10 variations of this architecture, each varying slightly in terms of face resolution, additional intermediate layers, and hardware requirements. The project is open-source, and is actively updated.
    
    \item \textbf{FaceSwap-GAN}: FaceSwap-GAN was created in 2018 as a fork of FaceSwap. It is owned by online user \textit{shaoanlu}. FaceSwap employs the exact same base neural architecture for face-swapping as FaceSwap, i.e. it employs two deep auto-encoders. An additional discriminator is added to provide an adversarial loss, as found in GAN's. A VGGFace perceptual loss is also added to improve image quality. The decoder also predicts a segmentation attention mask to eliminate artifacts and improve swap quality. FaceSwap-GAN is an open-source project, and is no longer updated. 
    
    \item \textbf{DeepFaceLab 1.0/2.0}: DeepFaceLab (DFL) was created in 2018 as a fork of FaceSwap. It is owned and maintained by online user \textit{iperov}. DFL employs the exact same base neural architecture for face-swapping as FaceSwap i.e. it employs two deep auto-encoders. DFL offers 4 variations of this architecture, each varying slightly in terms of face resolution, additional intermediate layers, and hardware requirements. DFL is an open-source project, and is actively updated.
    
    \item \textbf{DFaker}: Dfaker was created in 2018. It is owned by online user \textit{dfaker}. Dfaker employs the exact same base neural architecture for face-swapping as FaceSwap i.e. it employs two deep auto-encoders. Dfaker substitutes the use of MAE or SSIM reconstruction loss with the masked DSSIM loss. Dfaker also modifies the decoder to predict a segmentation mask (as in FaceSwap-GAN) to be used for demarcating the face-swapping area. Dfaker is an open-source project, and is no longer updated.
    
    \item \textbf{FakeApp}: FakeApp was created in 2018. It is owned and by online user \textit{deepfakeapp}. FakeApp employs an unknown neural architecture for face-swapping, but is rumoured to use the exact same base neural architecture as that of FaceSwap. FakeApp is a closed-source project, and is no longer updated.
    
    
    \item \textbf{MyFakeApp}: MyFakeApp was created in 2018 as a fork of FaceSwap. It is owned by online user \textit{radek}. MyFakeApp employs the exact same base neural architecture for face-swapping as FaceSwap i.e. it employs two deep auto-encoders. MyFakeApp is an open-source project, and is no longer updated.
    
    \item \textbf{(a) Deepfakesapp.online (b) Deepfakes web $\mathbf{\beta}$, (c) DeepFake.me}: These websites were created in 2018. They are owned by unknown users, and employ unknown neural architectures for face-swapping. All three websites use closed-source tools, and are purportedly actively updated.
    
    \item \textbf{Zao:} This mobile application was created in 2018. It is owned by a subsidiary company of Chinese software company Momo. Zao employs an unknown neural architecture for face-swapping, but is rumoured to a face animation technique known as GANimation. Zao is closed source and is \todo{actively updated - I need to check this.}
    
    \item \textbf{Reflect and Doublicat}: These mobile applications were created in 2018 and 2020, respectively. They are owned by Ukrainian company Neocortext/RefaceAI. Reflect and Doublica employ an unknown GAN-based neural architecture for face-swapping. Both applications are closed source and are actively updated.
    
    
\end{enumerate}
\noindent\textbf{Academic community.} \todo{brief intro to academic methods here.} \bimal{This part should be brief. we can discuss when we meet.}

\begin{enumerate}
    \item \textbf{FSGAN:} FSGAN was proposed at ICCV 2019 by Nirkin et al. FSGAN employs a tri-GAN neural architecture for face-swapping. The first component of FSGAN comprises a GAN that takes as input a heatmap of facial landmarks of the target face to be replaced, and an image of the source face to be swapped in. The output is a \textit{re-enacted} face, with the identity of the source, but the pose and expression of the target. This is achieved via a stepwise consistency loss, which iteratively performs the \textit{re-enactment}. The same generator also outputs a facial segmentation mask. This is achieved via a standard cross-entropy loss. The second component of FSGAN is an in-painting GAN that takes as input the re-enacted face and corresponding segmentation. It then outputs an estimate of missing parts of the face. This is achieved via a custom in-painting loss. The third and final component of FSGAN is a blending GAN, which blends the in-painted face into the target image. This is achieved via a custom poisson blending loss. All three components employed perceptual, reconstruction and adversarial losses. FSGAN is open-source.
    
    \item \textbf{Fast Face Swap CNN:} Fast Face Swap CNN was proposed at ICCV 2017 by Korshunova et al. Fast Face Swap CNN employs a CNN-based neural architecture for face-swapping. A CNN is trained to take as input a target image, and replace the facial identity in said image with a source face, which is predefined during training. Affine transformations are used to align all faces to a frontal view before feeding through the CNN, and to reverse the alignment change in the resulting output. The swap is achieved via a custom cosine loss. This loss attempts to match each patch of the input target image to the closest available patch in a group of available images of the source face. Other objective losses include a perceptual and light loss. Fast Face Swap CNN is open-source.
    \item \textbf{IPGAN:}
    \item \textbf{FaceShifter:}
    \item \textbf{FSNet:}
    \item \textbf{DF-VAE:}
\end{enumerate}

% \begin{itemize}
%     \item Begin with quick discussion origins of Deepfakes: see reddit user, uwashington obama video. Mention names of initial tools like FakeApp.
%     \item Talk about generative models i.e. the tech behind it - how it has evolved from CNNs and GANs and adversarial autoencoders and VAEs and whatnot. Talk about how generative media is a threat already in other domains as well (text, audio).
%     \item Move into references to major faceswapping Deepfakes in the news like nancy pelosi one.
%     \item Talk about proliferation about generation methods in community and academia. Then mention public efforts to catch them (Pentagon race against Deepfakes, DFDC).
%     \item Academia is thus pursuing it, talk about unsupervised/supervised efforts.
% \end{itemize}
\section{Deepfake Datasets}


\subsection{In-The-Wild Deepfake Dataset}
We present a dataset of Deepfake videos \textit{in-the-wild}, generated by the public Deepfake-generation community. To build this representative dataset, we gathered videos from two popular video hosting services - \textit{YouTube} and \textit{Bilibili\footnote{Widely recognized as a prominent video hosting website in China.}}. We then use semi-automated methods to verify that the gathered videos are indeed Deepfake videos. 

\bimal{We should have a table providing high level stats for each dataset. This includes number of videos, total number of frames, Total duration of all videos (hrs), avg. duration, avg. \#frames}

\bimal{Also give me an estimate of the total amount of storage used by the videos.}

\bimal{Another table should explain content in these videos. For each dataset, pick few videos with highest popularity (same based on vides), and provide their titles/description, median popularity and same, and lowest popularity and same.}

\subsection{Data Sources}
\subsubsection{YouTube}
We began gathering videos from popular video hosting platform, YouTube. In order to gather as many videos as possible, we recorded the uploading channel for each Deepfake video found (in lieu of the video itself). We began with a YouTube search, using keywords `Deepfake' and `faceswap', amongst many others\footnote{Other keywords/phrases included: \textit{synthetic videos, neurally generated videos, deep video, deepfacelab, fakeapp, fake video, artificially generated videos}. These keywords yielded no channels that had not already been revealed by \textit{Deepfake} and \textit{faceswap}.}. We recorded the channels revealed by the first 10 pages of search results. By clicking on each of these channels, we were also able to view and record related channel recommendations. Similarly, by clicking on the most-recent videos for these channels, we were able to view related videos and record the associated uploading channel. 

We also used Google Trends to view related Google search queries, with that could yield more YouTube channel content. For each of the search terms used in our initial YouTube search, we viewed related topics and keywords on Google Trends. We automated this process to record related keywords from 5 different geographical regions (USA, India, China, Russia, and Spain) using a proxy. However, these topics and keywords only referred to specific YouTube videos, the associated channel of which was already recorded.

We then turned to Reddit.com, which hosts two popular Deepfake discussion sub-forums, `GIF Fakes' and `SFWDeepfakes', to obtain listings for more YouTube channels. Other content-focused Reddit.com sub-forums, such as \textit{Politics}, have banned Deepfake content i.e. use democratically elected forum moderators who regularly remove such posts. In both of these sub-forums, we found that individual users had been uploading posts that linked to videos, either uploaded by themselves, or by another content creator. We thus scraped all posts for YouTube-related URLs. If the URL was a channel, we recorded it. Similarly, if the URL was a video, we reverse-traced the uploading channel and recorded it. Non-YouTube URLs led to platforms such as Reddit's own video-hosting service, Vimeo, and Imgur, all of which contained sparse amounts of novel Deepfake content, instead offering several duplicates of existing YouTube videos.

\subsubsection{Bilibili}
We began the Bilibili search with the keyword `zao', which refers to a popular mobile application that enables a user to swap their face into a movie clip. Zao, a free deepfake face-swapping app that’s able to place your likeness into scenes from hundreds of movies and TV shows after uploading just a single photograph, has gone viral in China. Other keywords, i.e. those used on the YouTube search, primarily revealed videos already available on YouTube, as well as instructional and reaction videos. We observed that nearly all uploading channels for these videos uploaded sparse amounts of Deepfake content. Consequently, we recorded the videos themselves (in lieu of the channels). We thus iterated through every page of search results, and recorded all the videos obtained. By clicking on these videos, we were able to view related videos, but did not obtain any videos not already returned in the original search results. Similarly, Reddit.com sub-forums yielded no Bilibili.com URLs. 

\subsection{Downloading and Filtering Data}
\subsubsection{YouTube}
We manually iterated through 195 recorded YouTube channels, discarding those that primarily uploaded non-Deepfake content. For each of 84 remaining channels, we analyzed metadata for each uploaded video. We accordingly automated the download of those videos of which the title or description contained keywords used in the original searches. A representative random sample of these videos was manually examined in order to ensure that such a filtering criteria was adequate. For each remaining video, we manually examined both the video as well as video metadata i.e. title, description and popular comments. We then downloaded those videos which we consequently deemed to be Deepfakes\mj{We need to elaborate on the methodology further. How do you establish a video to be deepfake? Did at least two people watch the video and agree on the manual labels? It might be helpful to add a separate subsection on "labeling" so that it is easily accessible to the reader}. A total of 1,062 Deepfake videos were thus downloaded from the channels of 84 YouTube channels primarily dedicated to Deepfake content creation.\mj{So if I am reading this correctly, these 84 Youtube channels appeared in the first ten pages of the Youtube search for the keywords "deepfake" and "faceswap"? (since you say other keywords did not return any more results). Why do we stop at ten pages? Is there more content to be found if we keep going?}

\subsubsection{BiliBili}
Each recorded Bilibili video was similarly subjected to an automated filtering, where only videos that contained `zao' in the title or description were downloaded. A representative random sample of these videos was also manually examined. A total of 984 Deepfake videos were downloaded from Bilibili.
\mj{Hmm, we are filtering before downloading. Later we analyze the popularity of the content - these metrics will be affected due to the filtering we are doing. So, it might be beneficial to collect everything, and filter videos that repeat later on, i.e., after we answer the question of how much content is out there. It will be interesting to see how much content is replicated too!}

\mj{Dataset description: I think it will also be nice to add summary statistics of the "claimed tools" by the video creators. I also want to know what category these videos were posted under (say for example, are ~50\% of these videos posted under tutorials/ how tos?)} 


\subsection{Existing Academic Datasets}
Recent work has proposed a variety of datasets to aid in the study of Deepfake and neurally generated media detection. We present a brief summary of these datasets below: \todo{Todo: for each dataset make sure to add a) avg duration b) associated generation method c) timeline of release/updating. d) number of videos in each class.}
\begin{enumerate}
    \item \textbf{Celeb-DF~\cite{celebdf}:} In 2020, Li et al. released a dataset containing 590 real videos from YouTube, and 5,639 Deepfake videos generated in-house, using an unknown, \textit{improved} generation method, with the goal of providing Deepfakes of quality similar to those available online.
    \item \textbf{DeepfakeTIMIT~\cite{deepfaketimit}:} In 2018, Korshunov et al. released a dataset containing 320 real videos of 10 subjects from the VidTIMIT dataset~\cite{VidTIMIT}, 320 low-quality Deepfake videos, and 320 high-quality Deepfake videos. The Deepfake videos were generated using the open-source tool, FaceSwap-GAN. 
    \item \textbf{FaceForensics++~\cite{ffpp}:} In 2019, Rossler et al. released a dataset containing 977 real videos from YouTube, and 1000 Deepfake videos generated using the open-source tool, FaceSwap.
    \item \textbf{DeepfakeDetectionChallenge~\cite{facebookdfdc}:} In 2019, Facebook released a dataset to accompany their \$1m Deepfake Detection Challenge. This dataset contains \todo{XXX} real videos and \todo{XXX} fake videos generated using 2 unknown Deepfake generation methods.
    \item \textbf{DeepFakeDetection~\todo{\cite{ffpp}}}: In 2019, Google and Jigsaw released a dataset containing over 363 real videos created in-house with 28 actors, and over 3000 Deepfake videos created using unknown Deepfake generation methods.
    \item \textbf{UADFV~\cite{UADFV}:} In 2018, Li et al. released a dataset containing 49 (unreleased) real videos from an unknown source, and 49 Deepfake videos generated using the now-extinct application, FakeApp.
    \item \textbf{DeeperForensics~\cite{deeperforensics}:} In 2020, Jiang et al. released a dataset containing 50,000 real videos created in-house with 100 actors, and 10,000 Deepfake videos generated using a custom method, DF-VAE. 
\end{enumerate}

% \subsection{Datasets}
% \subsubsection{Content categories}
% \begin{itemize}
%     \item Single person face-swapped, e.g., news clip, celebrity interview
%     \item Multi-person where one or more is swapped. Don’t know which face is swapped
%     \item Lip manipulations
% \end{itemize}


% \begin{itemize}
%     \item Discuss prior work on summarizing Deepfakes i.e. 3 studies at  \url{https://arxiv.org/abs/1909.11573} and at~\url{https://arxiv.org/pdf/2001.00179.pdf} and at \url{https://arxiv.org/pdf/2001.06564.pdf}
%     \item Then also talk about deeptracelabs - how they released a study in 2019, and weekly newsletters.
%     \item cite work on generation: cite FSGAN, RSGAN, etc. Do we mention community methods here?
%     \item cite some supervised methods
% \end{itemize}
\section{Analyzing In-The-Wild Deepfakes}
\mj{This argument needs to be revisited to flow with the theme of the paper.}To build tools that properly detect and defend against real world Deepfake use we must understand how Deepfakes in the wild are created, shared, and used. To that end we will be addressing questions around the current growth rate of online Deepfake content, how content is distributed among the creators, the engagement and spread of such content, and common situations defense techniques will encounter. \bimal{Do add billibili results to every subsection below.}

\subsection{Content Growth}
The key metrics for measuring \mj{sector seems off here}sector growth are the number of creators working on Deepfake content and the number of Deepfake video being uploaded. Figure~\ref{fig:channel_date} and figure~\ref{fig:video_date} show that both of these metrics saw a slight bump in January of 2018 with the original release of FakeApp, but the largest jump happened at the beginning of 2019 when DeepFaceLab and FaceSwap became popular open source alternatives to FakeApp. This growth is not simply a temporary spike either, the rate of growth has stayed consistent since the beginning of 2019 with 90\% of content having been released since then. \bimal{can you confirm whether the spile really corresponds to deepfacelab, and faceswap? you know the method associated with the video.}

\subsection{Content Creators}
We will be looking at two key indicators to understand the distribution of Deepfake content on YouTube: the number of subscribers channels have, which serves a representation of their reach, and the number of videos posted by each channel, a more direct measure of content location.

Figure ~\ref{fig:videos_channel} shows a notable top heavy skew in videos per channel with 60\% of all channels posting fewer than 10 videos and 20\% of channels posting only 1 or 2 videos. The majority of content (75\%) was created by only 8 channels. Figure ~\ref{fig:subs_channel} tells a similar story for channel subscriptions with the median number of subscribers being only 41
\bimal{can you also do analysis to find out who is driving the growth of deepfake content? is it the big players or the small players? You can look at fraction of videos produced by big players during the peak growth period or something like that.}


\subsection{Engagement and Popularity}
\mj{We also need to include a CDF plot of the number of views}
To quantify spread we looked at the ratio between views a given video receives and the number of subscribers the channel that posted that video has. Across YouTube a viewer to subscriber ratio of 1 to 10 is considered acceptable\mj{Please include citation for this. Also, try to see if we can get category specific numbers instead of the general numbers}. That is if a channel has 10,000 subscribers, they can expect 1,000 views on a new video they post. A high view to subscriber ratio implies that the content has spread beyond the audience of the channel and incredibly high ratios serve as indicators that a video has gone viral\mj{hmm I think we can make the same point only by number of views as well. I think we should use the ratio as a supplementary point for the argument of virality. Isn't it rather well-known that the videos are watched well beyond the subscribers of the channel?}. Figure~\ref{fig:sub_view} shows that Deepfake content has a notably large view to subscriber ratio with 60\% of Deepfake videos having a ratio of at least 1 to 1. This heavily implies that Deepfake content easily and often spreads beyond the audience of its channel and underscores the importance of proper defense and detection schemes.

The traditional measurement of engagement on YouTube consists of (Likes + Dislikes + Comments / Views) and serves as an approximation of how much of an impact a video had on the audience watching it. Across YouTube the average engagement hovers between 4\% and 5\%\mj{Again please add citation here}. Figure~\ref{fig:engagement} shows Deepfake content only manages a 1\% average engagement and only 15\% of Deepfake content have over 4\% engagement\mj{please explain how is the percentage engagement calculated?}. This implies that while the viewers that do watch Deepfake content view it passively, simply watching the video and moving on without engaging with traditional metrics. Together these points imply that the popularity of a Deepfake video has very little to do with the subscribed audience of the channel and instead much more to do with the video becoming widely shared. 
\mj{what are the max, min number of views seen for videos in our dataset? maybe also mention the titles or what was the deepfake about}

\subsection{Content Analysis}
\bimal{analyze duration, number of faces, number of fake faces, compression}
%\mj{We may like to move this to the dataset section. }\bimal{Mobin: i think it's better to put it here, because we will be comparing with academic dataset. i an explain.}
While Deepfake content is diverse there are still several categories we can break Deepfake videos into with different implications on detection. Broadly those categories are:
\begin{itemize}
    \item Single face faked the whole time
    \item Single face faked the whole time but not always present
    \item Single face faked for only part of the video
    \item Multiple faces, single face faked
    \item Multiple faces, single face faked for only part of the video
    \item Multiple faces, multiple fakes
\end{itemize}
The majority of content contains only a single face that is faked, and that face is present for only part of the video with multiple face fakes being exceedingly rare\mj{We need to say how we arrived at this. Was it via manual labeling? Can we define "majority" further?}.

\subsection{Deepfake Methods}
\bimal{we also need to compare with academic datasets}
We took a conservative approach to determining the method for Deepfake videos. Each video was manually visited and the description, title, and creator comments were checked to see if a method was stated. If none was stated then the video was marked as unknown. An important note is we have several examples of channels which used multiple methods to generate different videos so it would be irresponsible to assume that any channel used the same method for all videos. 

Figure~\ref{fig:methods_pie} describes the distribution of the three Deepfake technologies that we found on YouTube: FakeApp, FaceSwap, and DeepFaceLab. DeepFaceLab makes up the vast majority of videos for which we have a stated method (94\%), but an important note is that videos produced between 2018 and 2019 were most likely using FakeApp as FaceSwap and DeepFaceLab were not yet available.
\mj{Consider merging some of the plots in this section. They take a lot of real estate :) While I got a sense of the temporality and engagement of these videos, I could not get a sense of how many viewers are watching these videos? Are they popular? Are they a problem? }
\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Metadata_Figures/channel_date_distribution.png}
  \caption{Publish date of Deepfake channels}
  \label{fig:channel_date}
\end{figure}
\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Metadata_Figures/date_distribution.png}
  \caption{Publish date of Deepfake videos}
  \label{fig:video_date}
\end{figure}
\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Metadata_Figures/channel_sub_distribution.png}
  \caption{Subscribers per channel}
  \label{fig:subs_channel}
\end{figure}
\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Metadata_Figures/channel_video_distribution.png}
  \caption{Videos per channel}
  \label{fig:videos_channel}
\end{figure}
\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Metadata_Figures/engagement_distribution.png}
  \caption{Percentage of engagement}
  \label{fig:engagement}
\end{figure}
\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Metadata_Figures/view_sub_ratio.png}
  \caption{Ratio of views on a video to subscribers on the channel posting the video}
  \label{fig:sub_view}
\end{figure}
\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Metadata_Figures/generation_method_chart.png}
  \caption{Generation methods used on YouTube}
  \label{fig:methods_pie}
\end{figure}
\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Metadata_Figures/BiliBili_sub_distribution.png}
  \caption{Subscription distribution on BiliBili}
  \label{fig:bb_sub_dist}
\end{figure}
\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Metadata_Figures/BiliBili_video_distribution.png}
  \caption{Video distribution on BiliBili}
  \label{fig:bb_video_dist}
\end{figure}
\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Metadata_Figures/BiliBili_video_views_distribution.png}
  \caption{Video view distribution on BiliBili}
  \label{fig:bb_video_views}
\end{figure}


% \section{Fingerprinting Generators}
% \subsection{Fingerprinting performance}
% \subsection{Compare with research community datasets}

\section{Detecting Deepfakes}
\subsection{Detection performance}
\subsubsection{Supervised}
Some candidates here:\\(need to add more supervised methods)\\

MesoNet is a CNN-based DeepFake detection
method targeting on the mesoscopic properties of images. The model is trained on unpublished DeepFake
datasets collected by the authors.

Xception corresponds to a DeepFake detection method based on the XceptionNet model [12] trained on the FaceForensics++ dataset. 

CapsuleForensics Network uses capsule structures based on a VGG19 network as the backbone architecture for DeepFake classification. This model is trained on the FaceForensics++ dataset.

Multi-task is a recent DeepFake detection
method built on a CNN model that can simultaneously detect image manipulation and segment manipulated areas. The model is
trained on the FaceForensics dataset.

VA is another DeepFake detection method
aims to capture visual artifacts in the synthesized faces, areas such as eyes, teeth and facial contour. The work proposes two variants of the method: VA-MLP which is a multilayer
feedforward neural network classifier, and VA-LogReg based on a simpler logistic regression model. We compared the performance these two variants and chose the better one: VA-MLP. The model is trained on unpublished dataset, of which real
images are cropped from CelebA dataset and the
DeepFake videos are from YouTube.
\begin{itemize}
    \item CapsuleForensics networks\\
    (Code: \url{https://github.com/nii-yamagishilab/Capsule-Forensics-v2})
    \item MesoNet-4\\
    (Code: \url{https://github.com/DariusAf/MesoNet})
\end{itemize}
\subsubsection{Unsupervised}
Some candidates here:\\

FWA detects DeepFake videos using a ResNet-50 [19] to expose the face warping artifacts introduced by the resizing and interpolation operations in the basic DeepFake maker algorithm. This model is trained on self-collected face images.

 DSP-FWA is a recently further improved method based on FWA, which includes a spatial pyramid pooling (SPP) module [18] to better handle the variations in the resolutions of the original target faces. This method is trained on self-collected face images
\begin{itemize}
    \item Face Warping Artifacts(fake data simulation)\\
    (Code: \url{https://github.com/danmohaha/CVPRW2019_Face_Artifacts})
    \item Dual Spatial Pyramid for Exposing Face Warp Artifacts(fake data simulation)\\
    (Code: \url{https://github.com/danmohaha/DSP-FWA})
    
    \item faceX-ray(fake data simulation)\\
    (Code: unpublished, need to request)
    \item learning based noiseprint: Extracting camera-based fingerprints for video forensics\\
    (Code: unpublished, need to request)
\end{itemize}
\subsubsection{Other Methods}
Corporate any traditional forgery detection method? like splicing detection. [Detecting Photoshopped Faces by Scripting Photoshop] is a method for detecting one very popular Photoshop manipulation – image warping applied to human faces. Since deepfake videos have similar face warping artifacts, we use the trained model to detect video frames directly. The trained detection model estimates the manipulation probability of the input video frame. 
SpliceBuster is a new blind splicing algorithm to detect image splicing without any prior information. Local features are computed from the co-occurrence of image residuals and used to extract synthetic feature parameters. The algorithm will output a heat map (right) indicating the splicing part in correspondence with the ghost.
[] applies this self-consistency model to the task of detecting and localizing image splices. The proposed method obtains state-of-the-art performance on several image forensics benchmarks, despite never seeing any manipulated images at training.

\begin{itemize}
    % \item Idea 1: Aggregating fingerprints + SVM classifier
    % \item Idea 2: Learning-based fingerprint + SVM classifier
    % \item Idea 3: Supervised with transferabitlity
    \item Detecting Photoshopped Faces by Scripting Photoshop
    Code: $https://github.com/PeterWang512/FALdetector$
    \item Splicebuster: A new blind image splicing detector(traditional image-splicing detection) Code: $http://www.grip.unina.it/research/83-multimedia_forensics/100-splicebuster.html$
    \item Fighting Fake News: Image Splice Detection via Learned Self-Consistency(ECCV18) Code: https://github.com/minyoungg/selfconsistency

    
    
\end{itemize}
\subsubsection{Compare With Research Community Datasets}
\begin{itemize}
    \item UADFV
    \item DF-TIMIT
    \item FaceForensics++
    \item Deepfake detection dataset(Google and Jigsaw)
    \item Deepfake detection challenge(Facebook)
    \item DeeperForensics(SenseTime, new dataset)
\end{itemize}


\subsection{Discussion on Detection Performance}
\begin{itemize}
    \item Discuss performance of a representative set of methodologies on our dataset. 
    \item \textbf{Horizontal method-wise comparison.} Does one method work everywhere? Does every method fail somewhere?
    \item \textbf{Longitudinal dataset-wise comparison.} Choose the best 1/2/3 methods, and evaluate on both academic datasets and our in-the-wild dataset, and compare the performance.  Is there any gap between evaluation on our in-the-wild dataset and evaluation on academic benchmarks.
    \item Our own generalized detection alternative - do we present it here? Allude?
    
    
\end{itemize}

\subsection{Identifying fake regions}







% \subsubsection{Community Methodologies}
% \begin{itemize}
%     \item Encoder-Decoder: Summarize FakeApp, MyFakeApp, FaceSwap, DFaker, DeepFaceLab.
%     \item Encoder-Decoder + GAN: Summarize FaceSwapGAN, DeepFaceLab.
%     \item Points for discussion: variance in the loss function for reconstruction (sometimes MSSIM), performance with and without adversarial training (i.e. with and without the + GAN part.) Summarizing the 13 or so architectures available in DeepFaceLab.
% \end{itemize}
% \subsubsection{Academia Methodologies}
% \begin{itemize}
%     \item GAN: Summarize FSGAN, fast-face swap using CNN, RSGAN, IDPGAN.
%     \item Modified Encoder-Decoder: FaceShifter, FSNET
%     \item VAE: DFVAE
%     \item non-neural (optional?): Face2Face
%     Acknowledging that some of these methods are a kind of zero-shot (don't need to be trained on new faces). Emphasize different in architecture developments (encoder-decoder vs all of these) between community and academic works.
% \end{itemize}
% \subsection{Content Creators}
% \subsubsection{Deepfake Media in the Wild(Meta data)}
% Categorize them:\\
% \textbf{Big Players(XXX\%)}
% \begin{itemize}
%     \item What types of platforms is this content hosted on? (YouTube, Reddit, etc.) Distribution of content across platforms? The account region?
%     \item Popularity - subscriber count, views, number of videos, est. income, etc.
%     \item Is it possible to evaluate quality? The progress of quality? Longitudinal study of quality vs time?
%     \item Reverse engineer methods that generate Deepfakes?(This might evolve into a section later.)
% \end{itemize}
% \textbf{Small Players(XXX\%)}
% \begin{itemize}
%     \item Platforms?(YouTube, Reddit) The distribution on platforms? The account region?
%     \item Popularity - subscriber count, views, number of videos, est. income, etc. Are they creating new content or just spreading existing content?
% \end{itemize}

% \subsubsection{Academic datasets}
% \begin{itemize}
%     \item UADFV
%     \item DF-TIMIT
%     \item FaceForensics++
%     \item Deepfake detection dataset(Google and Jigsaw)
%     \item Deepfake detection challenge(Facebook)
%     \item DeeperForensics(SenseTime, new dataset)
% \end{itemize}


% \subsubsection{The Value of Deepfake in the wild}
% \begin{itemize}
%     \item provide new viewpoint of current existing Deepfakes from online(with our meta data) 
%     \item make it possible to explore the gap between academic benchmarks and real Deepfakes in the realistic world, because no user data has been used in any of benchmark dataset. If there is a gap. e.g., what are reasons causing the gap?
%     \item Test claimed state-of-the-art detection methods on real Deepfakes in the wild, and stand out the most effective one.
%     \item 
% \end{itemize}



% % \section{Deepfake Media in the Wild(Meta data)}
% % \subsection{Deepfake Content Hosting}
% % \begin{itemize}
% %     \item What types of platforms is this content hosted on? - Forums, video channels, datasets.
% %     \item What platforms are these? Distribution of content across platforms.
% % \end{itemize}

% % \subsection{Analyzing Deepfake Content}
% % \begin{itemize}
% %     \item Present dataset of Deepfakes gathered from aforementioned platforms?
% %     \item The progress of quality? Longitudinal study of quality vs time?
% %     \item Reverse engineer methods that generate Deepfakes?
% % \end{itemize}
% \subsection{Trace back the generation method}
% XXX

% \section{Detecting Deepfakes}
% \subsection{Existing methods}
% \subsubsection{Supervised methodologies}
% Just summarize. \\
% Some candidates here:\\
% \textbf{RNN based:}
% Deepfake Video Detection Using Recurrent Neural Networks;
% Recurrent Convolutional Strategies for Face Manipulation Detection in Videos.\\
% \textbf{Capsule networks:}
% Capsule-forensics: Using Capsule Networks To Detect Forged Images And Videos.\\
% \textbf{Visual artifacts:}
% Exploiting Visual Artifacts to Expose Deepfakes and Face Manipulations;
% Exposing Deep Fakes Using Inconsistent Head Poses.\\
% \begin{itemize}
%     \item FaceForensics++\\
%     (Code: \url{https://github.com/ondyari/FaceForensics})
%     \item Capsule networks\\
%     (Code: \url{https://github.com/nii-yamagishilab/Capsule-Forensics-v2})
%     \item MesoNet-4\\
%     (Code: \url{https://github.com/DariusAf/MesoNet})
% \end{itemize}




% \subsubsection{Unsupervised methodologies}
% Just summarize.\\
% Some candidates here:\\
% \begin{itemize}
%     \item learning based noiseprint: Extracting camera-based fingerprints for video forensics\\
%     (Code: seems unpublished, monitoring)
%     \item Face Warping Artifacts(fake data simulation)\\
%     (Code: \url{https://github.com/danmohaha/CVPRW2019_Face_Artifacts})
%     \item Dual Spatial Pyramid for Exposing Face Warp Artifacts(fake data simulation)\\
%     (Code: \url{https://github.com/danmohaha/DSP-FWA})
%     \item faceX-ray(fake data simulation)\\
%     (Code: empty github repository, monitoring)
% \end{itemize}




% \subsubsection{Discussion on detection performance}
% \begin{itemize}
%     \item Discuss performance of a representative sample of methodologies on our dataset. 
%     \item \textbf{Horizontal method-wise comparison.} Does one method work everywhere? Does every method fail somewhere?
%     \item \textbf{Longitudinal dataset-wise comparison.} Choose the best 1/2/3 methods, and evaluate on both academic datasets and our in-the-wild dataset, and compare the performance.  Is there any gap between evaluation on our in-the-wild dataset and evaluation on academic benchmarks.
%     \item 
%     \item Our own generalized detection alternative - do we present it here? Allude?
% \end{itemize}


% \subsection{Proposed Method}
% \begin{itemize}
%     \item Idea 1: Aggregating fingerprints + SVM classifier
%     \item Idea 2: Learning-based fingerprint + SVM classifier
%     \item Idea 3: Supervised with transferabitlity
% \end{itemize}

% \subsubsection{Detection performance of the proposed method}

\section{Conclusion}


